Complete Dictionary Learning via $\ell^4$-Norm Maximization over the Orthogonal Group

This paper considers the fundamental problem of learning a complete (orthogonal) dictionary from samples of sparsely generated signals. Most existing methods solve the dictionary (and sparse representations) based on heuristic algorithms, usually without theoretical guarantees for either optimality or complexity. The recent $\ell^1$-minimization based methods do provide such guarantees but the associated algorithms recover the dictionary one column at a time. In this work, we propose a new formulation that maximizes the $\ell^4$-norm over the orthogonal group, to learn the entire dictionary. We prove that under a random data model, with nearly minimum sample complexity, the global optima of the $\ell^4$ norm are very close to signed permutations of the ground truth. Inspired by this observation, we give a conceptually simple and yet effective algorithm based on "matching, stretching, and projection" (MSP). The algorithm provably converges locally at a superlinear (cubic) rate and cost per iteration is merely an SVD. In addition to strong theoretical guarantees, experiments show that the new algorithm is significantly more efficient and effective than existing methods, including KSVD and $\ell^1$-based methods. Preliminary experimental results on mixed real imagery data clearly demonstrate advantages of so learned dictionary over classic PCA bases.

==> cover.tex <==
\begin{center}
    \textbf{Cover Letter}
\end{center}
\begin{itemize}
    \item This submission is a extended version of a previous submission ``A Fast Holistic Algorithm for Complete Dictionary Learning via $\ell^4$ Norm Maximization'' to Signal Processing with Adaptive Sparse Structured Representations (SPARS) Workshop 2019 \url{http://www.spars-workshop.org/en/index.html}. We have improved 1) convergence result w.r.t. the objective function $\hat{f}(\mb A,\mb Y)$, previous submission to SPARS is a point-wise convergence result, current submission is a uniform convergence result with exponential rate of convergence; 2) convergence result w.r.t. the gradient of the objective function $\nabla_{\mb A}\hat{f}(\mb A,\mb Y)$, previous submission does not include this part; 3) More analysis of the proposed MSP algorithm, refer to section 4; 4) applications to more real world data, in this submission, we show the experimental result of our proposed algorithm on the MNIST dataset. 
    \item Yuexiang Zhai, Zitong Yang, Zhenyu Liao, John Wright, and Yi Ma are fully aware of this submission to JMLR.
    \item Recently collaborated action editors: Julien Mairal has collaborated with John Wright and Yi Ma in 2010.
    \item Editor Suggestions: David Wipf, Julien Mairal, Michael Mahoney
\end{itemize}
\newpage

\begin{center}
    \textbf{Review Reply}
    \begin{itemize}
        \item {\bf Review1:} This paper gives a new algorithm for complete dictionary learning problem. The new algorithm is based on the 4-th moment relaxation (which is closely related to the cumulant methods in independent component analysis). The main difference between this approach and previous approaches that are based on cumulants (especially those for ICA) is that the new algorithm finds all the d components simultaneously, by adding a constraint that makes sure all the components are orthonormal. The main result of the paper shows that the global optimal of the objective function will indeed give a good estimation of the true dictionary given enough samples. The paper also shows that ocally the objective function converges in a cubic rate (there are some concerns here, see below). Experimentally the new algorithm is very effective.

        Overall the new result is interesting. The new objective makes sense and is very effective in practice. While it would be nice to have a global convergence result, even the global convergence for n = 2 is not completely trivial. The paper should still address some of the concerns below:
        
        \rp{Thanks for your reviews. We have revised our paper according to some of your suggestions. In the meantime, we also made some clarification in the response.}
        
        \begin{itemize}
            \item \che 1. The paper needs to compare a bit more carefully with related work. In particular, some of the discussions (like cumulant methods for ICA or power iteration for tensor) are very related to the intuition for the algorithm, and should be mentioned when the algorithm is introduced. The method in this paper also rely fairly heavily on the Bernoulli-Gaussian model, and in particular the independence assumption for x. Some other sparse coding papers, including the SoS works, the work by Spielman et al. (although the proof requires indepence it's easy to relax the requirement), and works like https://arxiv.org/abs/1503.00778 or https://arxiv.org/abs/1310.7991 that work for lower sparsity levels, allow this independence assumption to be relaxed.\\
            \rp{Thanks for the suggestion. We have updated the paper accordingly. 1) We have added a paragraph that discusses the relationship between FastICA method and the MSP algorithm, please refer to the paragraph before Theorem 2; 2) We have added a paragraph (the paragraph after equation (3)) in our introduction to discuss https://arxiv.org/abs/1503.00778 and https://arxiv.org/abs/1310.7991.}
            \item \che 2. For finding all the component simultaneously, as the problem is effectively equivalent to a tensor decomposition problem (just by the cumulant method for ICA), it's worth talking about some tensor decomposition algorithms that find all components simultaneously. The most famous one is the alternating least squares (ALS) algorithm, which is very similar to the proposed algorithm except that it does not enforce the orthonomality constraint. There is also an objective with known global convergence properties (see https://arxiv.org/abs/1503.02101). I don't expect the ojective with known global convergence to perform well, but my experience has been that ALS converges fairly quickly for orthogonal tensor decomposition so it is worth comparing to ALS in the experiment section. \\
            \rp{Thanks for the comment, we have added\\ https://arxiv.org/abs/1503.02101\\ to our reference. As for ALS, we recognize that ALS method is mainly designed for orthogonal tensor decomposition and not for dictionary learning. Hence, we do not include such experiments for comparison.}
            \item \che 3. For Theorem 2, if I understand correctly, this theorem assumes that we are running the algorithm using the objective in expectation (or in other words using infinitely many samples). When there are only finite number of samples, there are two issues here: (1) The cubic convergence in Theorem 2 may no longer hold near the global minimum (which is a perturbed version of the global minimum at infinite samples); (2) Even if there is still cubic convergence, it's no longer clear why this is super important because anyway there is already a fixed accuracy loss in Theorem 1.\\
            \rp{Thanks for the comment. We could have written this part in a clearer manner. We have updated the introduction around theorem 2 and make it precise: 1) in the randomized MSP algorithm update (equation 11), the random matrix $(AY)^{\circ3}Y^*$ converges to its expectation and the expectation $( AY)^{\circ3}Y^*$ is highly related to $( AD_o)^{\circ3}D_o^*$, see proposition 10 and 11; 2) Theorem 2 is for the deterministic objective $\norm{AD_o}{4}^4$, not the randomized objective $\norm{AY}{4}^4$, the relationship between them is discussed in section 4.2. We have updated that part of the introduction for clarification.}
            \item There are also some minor issues that should be fixed:
            \begin{itemize}
                \item \che Please use citet and citep correctly, many of the citations should have been in parenthesis but are left in plain text.
                \\
                \rp{Thanks for the comment, we have updated all citation accordingly.}
                \item \che There are too many footnotes especially in the first few pages. It might be good to introduce the notations earlier and remove some of them.\\
                \rp{Thanks for the suggestion, we have removed around half of the footnotes accordingly and merged notations in the main body. }
                \item \che Page 8, paragraph below theorem 1, there shoudn't be a 1/p for the expectations.\\
                \rp{Thanks for the reminder, we have updated that paragraph accordingly.}
            \end{itemize}
        \end{itemize}
        \item {\bf Review2:} Summary:
        The paper considers the problem of learning a complete orthogonal dictionary from p data samples of dimension n. First, it proposes a l4-norm based constrained optimization program to learn the dictionary. It proves (Theorem 1) that under the Bernoulli-Gaussian data generating model (no additive noise) and given enough data samples, the proposed program recovers the ground-truth dictionary up to a signed permutation. Second, the paper also proposes a fixed-point-iteration-based algorithm called MSP (matching, stretching and projection). It proves (Theorem 2) that the algorithm converges locally in the sense that if the algorithm is initialized close to the ground-truth dictionary and ran on the expected objective, then it has cubic convergence (error is reduced from $\eps$ to $\eps^3$ in one iteration).
        
        Strengths:
1. l4-norm based constrained optimization program is proposed to solve the noiseless complete orthogonal dictionary learning problem.
2. It proves the identifiability of the dictionary using the proposed formulation under Bernoulli-Gaussian data model.
3. It proposes a new practical algorithm (MSP) to solve the l4-norm based optimization. And show its local convergence when the initialization is close enough.
Overall, under the Bernoulli-Gaussian data model, this paper is very good since it has an optimization formulation, an algorithm and proofs to show the algorithm works in large sample and with good initialization.  The only point is in question might be the practical applicability of the proposed method when the Bernoulli-Gaussian data model is not satisfied or when there is additive noise (to be explained in more details below).\\
\rp{Thanks for your insightful comments. As per your suggestion, we have updated the paper accordingly/provided reference to some other followup works, please refer to our response and the updated paper.}

There are also some minor contributions that are quite interesting for readers of interest, such as l2k norm formulation, relation between the proposed algorithm to the projected gradient ascent (PGA) in Section 4.2 and global convergence in dimension 2 in proposition 17.

Weaknesses:
\begin{itemize}
    \item \che In my opinion, the largest concern of the proposed method is its applicability to the real case where X is no longer Bernoulli-Gaussian and how to interpret the dictionary learned in this case. The proposed method (Equation 9) relies heavily on the Bernoulli-Gaussian data model. For example, Lemma 3, which is a key lemma to show that the population version of the objective finds the correct dictionary, heavily relies on the fact that each coordinate of $x_i$ is generated i.i.d. and with same variance. I think that if the coordinates of $x_i$ do not have the same variance, then additional adjustment on A is needed to recover the true dictionary.

    It would be great if the paper could at least have some empirical discussion on this matter, because many practical data will deviate from the Bernoulli-Gaussian model and it is helpful for practitioners to know how to adapt or how to interpret the results obtain under theoretical model.\\
    \rp{Thanks for the suggestion. Indeed, the proof relies heavily on the assumptions that all $x_i$ should have the same variance. However, our later experiments has demonstrated its capability of learning sparse representation from the MNIST dataset, which does not have the same (pixel-wise) variance. We have update the discussion in section 5.6 to address this issue. We believe this preliminary result can justify the empirical performance of the proposed algorithm and we would like to perform extensive empirical research of the MSP algorithm in the future.}
    \item \che The second concern is also pointed out by the authors in Section 6 that this paper does not cover the case with additive noise. It might be less important than the previous one, but again for the proposed method to be widely applicable, one might need to address this point at least empirically. Showing some empirical evidence about at what of amount of noise the proposed method starts to fail will be very helpful.\\
    \rp{Thanks for the comment. After this submission, we have found that the proposed MSP algorithm is robust to noise, sparse corruptions, and outliers, please refer to our later paper here:\\ https://openreview.net/forum?id=SJeY-1BKDS.
    }
    \item \che Experiments in Section 5.5, I understand the authors would like to compare with methods with some theoretical guarantees on the Bernoulli-Gaussian model. For general audience, is it possible to incorporate some comparisons with popular dictionary learning methods such as sparse coding, sparse PCA in SPAMS (http://spams-devel.gforge.inria.fr/). The SPAMS package should be quite fast in this case.
    \\
    \rp{Thanks for the suggestion, we have added experiments comparison with the SPAMS package in experiment 5.5, please find more details in table 2.}
    
    
\end{itemize}
    Other Comments:
    \begin{itemize}
        \item \che Comparison simulations with other methods in Section 5.5 are done in the sample size p much larger than dimension n case. 
        
        Is it possible to incorporate the case when p is close to the theoretical value about $\theta*n^2$?\\
        
        \rp{The purpose of comparison experiment is to demonstrate the efficiency and correctness of the proposed MSP algorithm, so we need to set the sample size $p$ large enough for the MSP algorithm to success. According to our analysis in Theorem 7 and Proposition 11, it is really hard to get the right constant of the sample complexity $\theta n^2$. We apologize for not providing the required experiment, due to such difficulty.}
        \item \che In Section 5.5, it claims "Within statistical errors, our algorithm gives slightly smaller values". Table 2 does not contain statistical errors. Is it possible to add the statistical errors by having multiple runs in Table 2?
        \\
        \rp{Yes, we have updated the paper accordingly.}
        \item \che In Section 5.4, theoretically, theta should be in linear relationship with p/n for fixed n, Figure 8(a) needs some comments about the obtained plot. \\
        \rp{Thanks for pointing this out. This inconsistency happens because of the constant C in theorem 7 depends on theta (actually we require $C>4/3\theta(1-\theta)$). Therefore, we may not directly observe a linear transition between $p$ and $\theta$ when $n$ is fixed. We have clarified this in the end of the second paragraph of section 5.4.}
        \item \che In Section 5.3, Figure 7(a) and 7(b) are interesting. There seems to be a trade-off between the choice of 2k and the number of samples available. Is there a recommendation for when to use L2k with 2k > 4?\\
        \rp{Thanks for the question, we currently do not have more results on balancing the rate of convergence and the sample complexity. The only conclusion we can draw about the l2k norm is that l4 seems to require the least sample complexity. We would like to leave the discussion of "rate of convergence verses sample complexity" in Figure 7 as future works.}
    \end{itemize}
    Also, according to the logic in this paper, it seems that 2k=3 should also be a good formulation, maybe even better than the case 2k=4. Can the simulation of 2k=3 be added? \\
    \rp{Thanks for pointing this out, a followup paper\\ (https://arxiv.org/abs/2002.10043) has already discussed the 2k=3 case thoroughly. We have included discussion about that work (also the 2k=3 case) in section 5.4 and the discussion section 6.}\\
    Writing needs to be improved:
    \begin{itemize}
        \item \che Page 9 Section 1.3.3, the two types of symmetry are not well defined. What is the definition of the continuous symmetry on Page 9?\\
        \rp{We apologize for the confusion, the continuous symmetry is referring to the symmetry of the discrete signed permutation group SP(n) over the continuous group O(n, R). We have removed the term "continuous symmetry" in the paper to avoid such confusion.}
        \item \che Current statement of Theorem 2 in Page 9 is confusing.
        
        First, it should bed stated that Theorem 2 is an informal version of Theorem 16. Second, even it is informal, it should not make false claims. Because Theorem 16 only proves results for MSP Algorithm 1 which is applied on the population version of the objective and different to MSP Algorithm 2 which is applied on the sample version, this statement needs to be more precise about it.  Also, up to page 9, it is not clear yet what a theorem about the optimum Identity matrix is relevant for general $D_0$. Please explain. \\
        \rp{Thanks for the comment. We could have written this part in a clearer manner. We have updated the introduction around theorem 2 and make it precise -- theorem 2 is for the deterministic objective $\norm{AD_o}{4}^4$, not the randomized objective $\norm{AY}{4}^4$, the relationship between them is discussed in section 4.2. Moreover, we have clarified the ``optimum to identity matrix'' in theorem 2 and added reference to different sections.}
        \item \che The reduction to the identity discussion in Section 4 is not clear.
        
        "the objective g(.) is invariant over O(n; R)", in what sense it is invariant?
        
        I roughly understand the "without loss of generality" argument but the current reduction is not rigorous.\\
        \rp{Thanks for the comment, we have updated the first few paragraphs of section 4 and provide more rigorous discussion that characterizes the "invariant".}
        \item \che Reference to experiments are needed in some places.
        
        For example, Page 8 before-last paragraph "As our analysis and experiments will show"; Page 11 Section 2.2. "our experiments will show" not sure how it is shown; Page 14 before Example 1 "Our analysis later will", which theorem is it referring to?\\
        \rp{Thanks for the thoughtful comment, we have updated the corresponding reference.}
        \item \che The citation style is not conform with that of JMLR. This deteriorates the reading experience in for example Page 4 and Page 5. \\Please refer to  (http://www.jmlr.org/format/format.html)\\
        \rp{Thanks for the suggestion, we have updated the citation accordingly. }
        \item \che In the same JMLR format requirement above, JMLR "encourage authors to use footnotes sparingly". Notation like footnote 13 and 15 should be put into notations paragraph in the main text. \\
        \rp{Thanks for the suggestion, we have removed around half of the footnotes accordingly and merged notations in the main body. }
    \end{itemize}
    Overall, based on the main contributions mentioned above, I suggest "accept after minor revision". At least, the writing needs be improved to cause no confusions. It would be great if some weakness points could also be addressed.
\end{itemize}

\end{center}

\newpage
